nnInteractive: Redefining 3D Promptable Segmentation

Accurate and efficient 3D segmentation is essential for both clinical and research applications. While foundation models like SAM have revolutionized interactive segmentation, their 2D design and domain shift limitations make them ill-suited for 3D medical images. Current adaptations address some of these challenges but remain limited, either lacking volumetric awareness, offering restricted interactivity, or supporting only a small set of structures and modalities. Usability also remains a challenge, as current tools are rarely integrated into established imaging platforms and often rely on cumbersome web-based interfaces with restricted functionality. We introduce nnInteractive, the first comprehensive 3D interactive open-set segmentation method. It supports diverse prompts-including points, scribbles, boxes, and a novel lasso prompt-while leveraging intuitive 2D interactions to generate full 3D segmentations. Trained on 120+ diverse volumetric 3D datasets (CT, MRI, PET, 3D Microscopy, etc.), nnInteractive sets a new state-of-the-art in accuracy, adaptability, and usability. Crucially, it is the first method integrated into widely used image viewers (e.g., Napari, MITK), ensuring broad accessibility for real-world clinical and research applications. Extensive benchmarking demonstrates that nnInteractive far surpasses existing methods, setting a new standard for AI-driven interactive 3D segmentation. nnInteractive is publicly available: https://github.com/MIC-DKFZ/napari-nninteractive (Napari plugin), https://www.mitk.org/MITK-nnInteractive (MITK integration), https://github.com/MIC-DKFZ/nnInteractive (Python backend).

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%alternative opening not directly focusing on SAM but on clinical usabillity
Accurate and efficient medical image segmentation is crucial for clinical tasks such as tumor delineation for radiation therapy, organ segmentation, and surgical planning.While essential for treatment, this process is extremely time-consuming and costly due to the required expertise of a highly skilled clinician. 
%Hence, various fully automated methods were developed~\citep{isensee_nnu-net_2021,mednext,huang2023stunet}, but they require supervision of a clinician and, in case of undesired outcomes, need laborious manual corrections.
Hence, various fully automated methods have been developed~\citep{isensee_nnu-net_2021,mednext,huang2023stunet}, but they remain restricted to the specific target structures they were trained on. Moreover, these methods may fail in real-world scenarios, particularly on images outside their training distribution, requiring human supervision and, in cases of undesired outcomes, necessitating laborious manual corrections.
\\ Interactive foundation models, like the Segment Anything Model~\citep{segment_anything},  promise to solve these issues by supporting users in segmenting any structure of their choice more efficiently. This spurred great interest in leveraging Interactive Foundation Models for medical imaging.
%In the medical domain, this can enable clinicians to create and refine segmentations with great efficiency through AI-assisted annotation, reducing overall time and cost required for manual annotation.
%This promise has spurred great interest in leveraging Interactive Foundation Models for medical imaging. %Interactive Foundation models like the Segment Anything Model (SAM)\cite{segment_anything} have transformed natural image segmentation by enabling flexible, prompt-based segmentation across diverse visual domains.
While SAM's direct application to medical imaging has shown promise \cite{roy2023sammd}, its lack of focus on medical imaging has driven a plethora of advancements, adapting interactive segmentation methods to the medical domains~\cite{medsam, cheng2023sammed2d, scribbleprompt, rokuss2025lesionlocator}.  %Using interactive prompting with points and bounding boxes enhances flexibility and overcomes traditional task-specific supervised models constrained by specific training distributions~\cite{isensee_nnu-net_2021, swinunetr, mednext, medsegdiff, multitalent}, limiting their generalizability across medical imaging tasks.\\


% Interactive Foundation models like the Segment Anything Model (SAM)~\cite{segment_anything} have transformed natural image segmentation by enabling flexible, prompt-based segmentation across diverse visual domains. 
% While SAM's direct application to medical imaging has shown promise~\cite{roy2023sammd}, it has also driven adaptations tailored for medical domains~\cite{medsam, cheng2023sammed2d, scribbleprompt, rokuss2025lesionlocator}. Using interactive prompting with points and bounding boxes enhances flexibility and overcomes traditional task-specific supervised models constrained by specific training distributions~\cite{isensee_nnu-net_2021, swinunetr, mednext, medsegdiff}, limiting their generalizability across medical imaging tasks.\\

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/figure1_method.png}
\end{center} 
\caption{Cool example images showing diversity and new prompts}
\label{fig:the_real_figure_1}
\end{figure}


\noindent Despite these advancements, existing interactive methods face significant limitations: \begin{enumerate*}[label=\roman*)]
    \item Methods operate on individual 2D slices,  neglecting the true volumetric nature of the data which can lead to segmentation inconsistencies across adjacent slices. Moreover, this leads to a lack of real-world applicability when wanting to create 3D segmentations as each slice needs to be prompted separately~\cite{medsam,cheng2023sammed2d,scribbleprompt}. 
    \item The methods that do support 3D volumes are often not generalists, typically trained on single imaging modalities like computed tomography (CT)~\cite{segvol, vista3d}, or
    \item are restricted to segment only a closed-set of target structures, limiting utility to only the classes seen during training~\cite{vista3d}. As a result, models struggle to generalize to unseen objects and to resolve ambiguities (e.g., distinguishing a kidney with and without a tumor). This violates the expected generalizability of foundation models and leaves them ill-equipped to handle unseen data. 
    \item Furthermore, most methods are constrained to simple but intuitive prompts such as points or 2D bounding boxes~\cite{3dsamadapter,medsam} with the exception of~\citet{scribbleprompt} which introduces 2D scribbles.
    Conversely, methods that work in 3D often introduce cumbersome and unintuitive prompts such as 3D bounding boxes.
    None of the current methods bridges the crucial gap of leveraging intuitive and simple 2D interactions to generate 3D segmentations, which could greatly enhance usability and efficiency for medical image annotation. 
    \item Not all models support negative interactions or iterative refinement, which is a necessary aspect for an interactive segmentation tool. Many that do support negative prompts limit them to points instead of providing all negative prompt types. %While some approaches explore more complex interactions, such as scribbles, these are so far limited to 2D applications~\cite{scribbleprompt}
    \item Finally, usability remains a major concern as current solutions lack intuitive interfaces, hindering their adoption in real-world use-cases where precision, flexibility, and ease of use are essential. 
\end{enumerate*}\\
%To date, no method exists that provides a unified approach to 3D interactive open-set segmentation, supporting a full spectrum of prompts—including positive/negative points, scribbles, bounding boxes, and novel interaction paradigms—across multiple imaging modalities.\\
%Existing 3D segmentation methods, on the other hand, rely on 3D-specific prompts such as 3D bounding boxes, which are often cumbersome and unintuitive to create. 
%Instead, leveraging intuitive 2D interactions for the 3D domain would significantly enhance usability and efficiency for medical image annotation.
%Furthermore, no 3D segmentation tool comprehensively supports both positive and negative interactions across all prompt types. 

%vorschlag um nicht so oft das gleiche zu sagen
\noindent In this work, we introduce \texttt{nnInteractive}, the first framework for promptable and interactive medical image segmentation that addresses all these issues. Rather than focusing on architectural innovations, our approach provides an all-in-one solution that systematically tackles critical challenges in interactive segmentation, including interaction diversity, positive/negative prompting, usability, and computational efficiency. A key aspect of our framework is the integration of an unprecedentedly large and multimodal 3D dataset containing 64,518 Volumes from over 120 public datasets spanning XYZ target structures.

%\noindent In this work, we introduce \textit{nnInteractive}, a novel framework for promptable and interactive medical image segmentation that comprehensively addresses these shortcomings. This paper does not focus on introducing methodological network novelty, as is often expected. Instead, it presents a comprehensive, all-in-one solution that addresses all the critical limitations of existing promptable models for medical imaging. Our work systematically addresses key challenges in interactive medical image segmentation, including interaction diversity, positive/negative prompting, usability, and computational efficiency, while incorporating an unprecedentedly large and multimodal 3D dataset.
\noindent Additionally, we provide a fully functional and user-friendly segmentation tool, integrated into the widely used Napari~\cite{napari} viewer and MITK Workbench~\cite{MITK}, facilitating seamless research and annotation workflows. Through extensive evaluation, we demonstrate that our approach establishes a new state-of-the-art in 3D interactive segmentation, setting a new benchmark for adaptable and user-centric medical image analysis.

\subsection*{Key Contributions}
\begin{itemize}
    \item The first 3D interactive open-set segmentation model, featuring negative/positive point, scribble, and box prompts, trained on CT/MR/PET/....
    \item Present an unprecedented scale with over 120 3D datasets, surpassing all competitors.
    \item Usable tool in well known Napari Image Viewer and MITK Workbench
    \item New type of interaction (lasso, initial seg) and supervoxels
    \item Focus on 3D: No tool supporting negative prompts so far. No tool with emphasis on user-friendlyness: 2D bounding boxes for a 3D segmentation. Big keyword: 3d from 2d interactions
    \item Holistic set of interactions, all interaction types supported (+ new ones) and all also supported in positive/negative refinement steps 
    \item unprecedented dataset scale with new modalities.
    \item Explicitly mention the "limited architectual novelty" but refer to original nnUNet paper, (transformer vs CNN - revisited) and carefully/well executed work.
    \item Early prompting since no good pre-trained (foundation style) encoders in medical (for 3D)
    \item Solution to patching: prediction propagation. Other mitigation strategies: none (predict patch only), downscale (scribbleprompt), zoom in zoomout. None of the others work. 192 resenc is sota so its fine to do dynamic sliding window
    \item Zero shot refinement of a given 3D seg; 3d from 2d slice; 3d from set of orthogonal 2d slices
\end{itemize}

==> sec/old_text_dump.tex <==
\section{methods}

\subsection{network arch}
%\noindent A key innovation of nnInteractive lies in its prompt integration strategy. Conventional interactive segmentation models~\cite{segvol, sammed3d, sam2, segment_anything, medsam, cheng2023sammed2d} first encode images and incorporate user prompts at the latent feature level via fusion mechanisms. While effective in 2D models pretrained on large-scale datasets, this approach is suboptimal for 3D medical imaging, where no large-scale foundation models exist. In foundation models, object concepts are already encoded in the latent space, allowing prompts to efficiently retrieve structures post-embedding. Although fine-tuning remains necessary, the model benefits from pre-learned object representations, simplifying adaptation and reducing the need to infer task-relevant structures from raw data.
%In contrast, models trained from scratch lack pre-established object representations, making structure isolation more difficult without early guidance. If prompts are introduced only after embedding, the model must first learn a general feature space without knowing which structures are relevant to the segmentation task, significantly increasing training complexity. Instead, we adopt early prompting, embedding user inputs as additional channels before feature extraction. This ensures that prompts influence the entire feature extraction process, allowing the model to learn task-relevant structures from the first layer onward.

% \noindent A key strategy of nnInteractive is its early prompt integration. While effective in 2D models pretrained on large-scale datasets, the conventional approach~\cite{segvol, sammed3d, sam2, segment_anything, medsam, cheng2023sammed2d} of incorporating user prompts after image encoding at the latent feature level is suboptimal for 3D medical imaging, where no large-scale foundation models exist. In contrast, we embed user inputs as additional channels before feature extraction, ensuring prompts influence the entire feature extraction process. This allows the model to learn task-relevant structures from the outset.


USER SIMULATION

%User interactions are dynamically simulated based on the model’s current prediction, ground truth, and the interaction strategy selected by the corresponding agent. Interaction simulation is describes in Appendix~TODO. By incorporating these distinct strategies, nnInteractive learns to adapt to different user behaviors, ensuring robust segmentation performance across a range of interactive refinement styles.

\subsection{Ambiguity}

% Interactive segmentation methods must dynamically adapt to user inputs and segment structures according to user intent. In many cases, the desired segmentation outcome is ambiguous. For example, in liver and liver tumor segmentation, users may want to segment either the liver with the tumor included, just the tumors or the liver without the tumors. Similarly, in cardiac cine-MRI, the left ventricle may be segmented with or without its lumen. Such ambiguities pose challenges for models trained in a strictly supervised fashion, as they are often constrained to predefined class distinctions. For instance, SegVol does not allow segmentation of the kidney together with a kidney tumor, as it was trained to always separate these classes.

% To address this, nnInteractive is explicitly trained to handle ambiguous labels. For datasets where multiple valid segmentations exist, we randomly sample label variations during training, showing realistic combinations of anatomical structures as target objects. This approach ensures that nnInteractive learns to resolve ambiguities based on user interactions, enabling flexible adaptation to different segmentation requirements. We furthermore make no efforts on harmonizing class definitions between datasets.


\subsection{interactions}

% \paragraph{Point Interactions.}
% Point interactions provide a corrective cue within the selected error region $V$. A Euclidean distance transform $D: \Omega \to \mathbb{R}$ is computed on $V$ and normalized to $[0,1]$, assigning the highest values to central voxels. Points are sampled using two strategies: a center-biased approach with $\alpha=8$ and a uniform sampling approach with $\alpha=1$, defining the sampling probability as
% \[
% p(x) = \frac{D(x)^\alpha}{\sum_{z \in V} D(z)^\alpha}.
% \]
% A spherical region of fixed radius 4 is placed around the sampled point and processed via a Euclidean distance transform, yielding a soft mask with intensities in $[0,1]$ peaking at the center.



% \paragraph{Bounding Box Interactions.}
% Building upon the previously described 2D slice extraction, the bounding box interaction operates on the extracted error region $S \subset \mathbb{R}^2$. To introduce variability, the bounding box is perturbed using three augmentations, each applied with probability 0.5: jittering, shifting, and scaling.

% Jittering independently perturbs each boundary by an offset sampled from $\mathcal{U}(-0.05, 0.05) \cdot d$, where $d$ is the corresponding bounding box dimension. Shifting translates the entire bounding box along each axis by an offset sampled from the same range. Scaling applies independent scaling factors $s \sim \mathcal{U}(0.8, 1.2)$ per dimension, with uniform scaling across dimensions enforced with probability 0.3.




% \paragraph{Lasso Interactions.}
% A lasso interaction provides a more precise alternative to bounding boxes by enclosing the selected 2D error region $S \subset \mathbb{R}^2$ within a flexible contour. To construct the lasso mask $L: S \to \{0,1\}$, we first generate a coarse enclosure of $S$ by applying morphological operations—closing and dilation—with structuring element sizes determined relative to the object thickness, measured by the directional Euclidean distance transform.

% This preliminary mask is then warped using a random deformation field $W$, where the deformation magnitudes along each axis are scaled proportionally to the corresponding directional EDT.



% \paragraph{Scribble Interactions.}
% Let $S\subset\mathbb{R}^2$ denote the extracted error region, and let $\{T_i\}_{i=1}^2$, with $T_i: S\to [0,\infty)$, be the directional Euclidean distance transforms computed on $S$, quantifying object thickness along each axis. Inspired by ScribblePrompt~\cite{scribbleprompt}, our method generates three types of scribble interactions—center, line, and contour scribbles—each selected with probability $\frac{1}{3}$. We introduce key improvements, ensuring constant scribble width and automatically scaling deformation parameters according to object size.

% Each scribble type follows a structured process: an initial line representation $L_{\mathrm{init}}$ is generated, deformed, and then reprocessed to ensure geometric consistency.

% \begin{itemize}
%     \item \textbf{Center Scribbles:} Compute the skeleton $\operatorname{sk}(S)$ and apply a random truncation operator $\mathcal{R}$ to simulate partial annotation:
%     \[
%     L_{\mathrm{init}} = \mathcal{R}\bigl(\operatorname{sk}(S)\bigr).
%     \]
%     \item \textbf{Line Scribbles:} Select two random points in $S$ and connect them with a straight line.
%     \item \textbf{Contour Scribbles:} First, erode $S$ with a radius proportional to object thickness (from $\{T_i\}$) to obtain $E_1(S)$, then erode again with a radius of 1 to extract the contour. The initial scribble is obtained by applying a truncation operation $\mathcal{R}$:
%     \[
%     L_{\mathrm{init}} = \mathcal{R}\bigl(E_1(S) \setminus E_2(S)\bigr).
%     \]
% \end{itemize}

% \noindent The initial scribble $L_{\mathrm{init}}$ is then warped via a random deformation field $W$, where the deformation magnitude is modulated by the directional EDTs $\{T_i\}$:
% \[
% L_{\mathrm{def}} = W\bigl(L_{\mathrm{init}}; \{T_i\}\bigr).
% \]
% Finally, $L_{\mathrm{def}}$ is skeletonized and dilated using a fixed structuring element $D_r$ (radius $r$) to ensure constant thickness:
% \[
% L = D_r\Bigl(\operatorname{sk}(L_{\mathrm{def}})\Bigr).
% \]
% This formulation enables realistic scribble interactions that serve as precise corrective cues for segmentation refinement.



ZOOM
% One major limitation of 3D models is that, due to VRAM constraints, images need to be processed in a patch-wise manner. If this is not accounted for, objects larger than the patch size cannot be properly segmented, causing the predictions to be cut-off at the patch borders. Most existing 3D methods do not propose solutions for this or rely on additional interactions to prompt new patch predictions until the object of interest is covered~\cite{vista3d, sammed3d} (FIG?). To handle this issue SegVol~\cite{segvol} has introduced a 'zoom in zoom out' strategy to aggregate global and local information by first predicting on a coarse resolution. SegVol agressively resizes the image to its patch size of 32x256x256, followed by sliding window refinement on full resolution.

% We build upon this idea by introducing an auto zoom algorithm (see \ref{fig:autozoom}). Starting from an initial zoom factor, nnInteractive detects whether the prediction touches the border of the currently visible ROI and iteratively zooms out by a factor of 1.5 until the object of interest fully fits into the ROI (max zoom out factor is 4). The predicted mask is then resized to the original image resolution and a sliding window refinement is performed on the mask. To ensure informed decisions by the model, the order in which the refinement patches are visited is optimized using a Dijkstra-like algorithm. Starting from the patch with the most guidance (i.e. the most predicted voxels), nnInteractive recursively visits the next most informative neighboring patches until all patches have been predicted.This ensures that the model starts predictions from the most informative region and incrementally extends to less constrained areas, leveraging its own previous predictions for consistent refinement. 
% The initial zoom factor is determined by the interaction that triggers it. It is determined such that the interaction is covered by the ROI in its entirety plus a border of 1/6th patch size in each dimension. 
% This dynamic scheme enables nnInteractive to invest only the compute that is really needed. For small objects, no zooming will be performed causing fast inference times. Larger objects, such as for example the liver, require more zoom and refinement.
% Our approach offers several key advantages over the fixed zoom used by SegVol: 0) It zooms exactly as much as is needed to cover the structure of interest, keeping relevant details in the segmentation output and optimally guiding the refinement patch 1) It avoids unnecessarily coarse downsampling which may be detrimental for small objects, 2) ensures compatibility with large images where global resizing would exceed VRAM capacities.

% Since bounding boxes and lasso share the same input channel in nnInteractive and bounding boxes of large objects may cause misleading signals at their edges, we convert positive bounding boxes to lasso prior to the refinement step. This ensures no false positive predictions are being made outside the object of interest.





\begin{table*}[]
\begin{tabular}{lcccccccc|c}
\hline
 \multirow{2}{*}{Model}                                      &\multirow{2}{*}{\shortstack{Native\\3D}}& \multicolumn{4}{c}{Prompt Types} & \multirow{2}{*}{Interactive} & \multirow{2}{*}{Open Set} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Different\\ Modalities\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}User-friendly\\ Tool\end{tabular}} \\
&& Point   & Box   & Scribble& Lasso  &                              &                           &                                                                                 &                                                                               \\

\hline
SAM~\cite{segment_anything}          &\emoji{cross-mark}      & \emoji{check-mark-button}       & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{cross-mark}      & \emoji{check-mark-button}                            &                           \emoji{check-mark-button}                            &                                                                                 \emoji{cross-mark}                            &                                                                               \emoji{check-mark-button}       \\
SAM-Med2D~\cite{cheng2023sammed2d}    &\emoji{cross-mark}      & \emoji{check-mark-button}       & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{cross-mark}      &                              \emoji{check-mark-button}                            &                           \emoji{check-mark-button}                            &                                                                                 \emoji{check-mark-button}                            &                                                                               \emoji{check-mark-button}       \\
MedSAM~\cite{medsam}                  &\emoji{cross-mark}      & \emoji{cross-mark}       & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{cross-mark}      &                              \emoji{cross-mark}      &                           \emoji{check-mark-button}                            &                                                                                 \emoji{check-mark-button}                            &                                                                               \emoji{cross-mark}                            \\
ScribblePrompt~\cite{scribbleprompt}  &\emoji{cross-mark}      & \emoji{check-mark-button}       & \emoji{check-mark-button}     & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{check-mark-button}                            & \emoji{check-mark-button}                         & \emoji{check-mark-button}                                                                               & \emoji{check-mark-button}                                                                             \\  SAM2~\cite{sam2}                      &2D+$t$& \emoji{check-mark-button}       & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{cross-mark}      & \emoji{check-mark-button}                            &                           \emoji{check-mark-button}                            &                                                                                 \emoji{cross-mark}                            &                                                                               \emoji{check-mark-button}       \\  SAM-Med3D~\cite{sammed3d}             &\emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{cross-mark}     & \emoji{cross-mark}      & \emoji{cross-mark}      & \emoji{cross-mark}                            &                           \emoji{check-mark-button}                            &                                                                                 \emoji{check-mark-button}                            &                                                                               \emoji{cross-mark}                            \\
NVIDIA VISTA~\cite{vista3d}                 &\emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{cross-mark}     & \emoji{cross-mark}      & \emoji{cross-mark}      & \emoji{check-mark-button}                            &                           \emoji{cross-mark}                            &                                                                                 \emoji{cross-mark}                            &                                                                               \emoji{check-mark-button}       \\
SegVol~\cite{segvol}                  &\emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}     & \emoji{cross-mark}      & \emoji{cross-mark}      & \emoji{cross-mark}                            &                           \emoji{check-mark-button}                            &                                                                                 \emoji{cross-mark}                            &                                                                        
\emoji{check-mark-button}       \\
\hline
 nnInteractive& \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       & \emoji{check-mark-button}       &\emoji{check-mark-button}       \\\end{tabular}
\end{table*}
